ClipFlip : Multi-view Clipart Design

We present an assistive system for clipart design by providing visual scaffolds from the unseen viewpoints. Inspired by the artists' creation process, our system constructs the visual scaffold by first synthesizing the reference 3D shape of the input clipart and rendering it from the desired viewpoint. The critical challenge of constructing this visual scaffold is to generate a reference 3Dshape that matches the user's expectation in terms of object sizing and positioning while preserving the geometric style of the input clipart. To address this challenge, we propose a user-assisted curve extrusion method to obtain the reference 3D shape.We render the synthesized reference 3D shape with consistent style into the visual scaffold. By following the generated visual scaffold, the users can efficiently design clipart with their desired viewpoints. The user study conducted by an intuitive user interface and our generated visual scaffold suggests that the users are able to design clipart from different viewpoints while preserving the original geometric style without losing its original shape.

==> questionnaire.tex <==
\section{Interview questionnaire}
In this section, we provide all the questions we asked in our interview questionnaire.
In the questionnaire, there are three sections, including user's drawing experience, the viewpoint survey, and the scaffold aids survey.

\subsection{User's drawing experience}
\begin{enumerate}
    \item Do you have any drawing experiences?
    \begin{enumerate}
        \item digital painting
        \item physical painting
        \item no
    \end{enumerate}
    \item If yes, for how many years?
\end{enumerate}

\subsection{Viewpoint survey}
\begin{enumerate}
    \item Do you think there are differences of drawing difficulties when you draw different the clipart under different viewpoints?
    \begin{enumerate}
        \item yes
        \item no
    \end{enumerate}
    \item If yes, which viewpoint you think is the most difficulty for airplane clipart?
    \begin{enumerate}
        \item front
        \item side
        \item top-side
    \end{enumerate}   
    \item If yes, which viewpoint you think is the most difficulty for chair clipart?
    \begin{enumerate}
        \item top
        \item side
        \item top-side
    \end{enumerate}   
\end{enumerate}
\subsection{Scaffold aids survey}
\begin{enumerate}
    \item Do you think visual scaffold is helpful for drawing novel view clipart?
    \begin{enumerate}
        \item yes
        \item no
    \end{enumerate}
    \item If yes, how the provided visual scaffold affect you while drawing? (open question)
    \item Other comments and suggestions. (open question)
\end{enumerate}

==> user_result.tex <==
\section{All Results of User Study}
% \iccmt{Add comparison to TBN on every cases}
We show all the design clipart from the participants of our user study, including two object categories, i.e., chair and airplane.

\subsection{Chair case1}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub01-result-clean.pdf}
    \caption{We show participant 01's result from (a) top, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 8:38 mins (top), 10:29 mins (side), and 27:10 mins (upper $45^{\circ}$) drawing without visual scaffold, and 2:39 mins (top), 6:15 mins (side), and 8:00 mins (upper $45^{\circ}$) with visual scaffold.
    }
    \label{fig:result-01}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub09-result-clean.pdf}
    \caption{We show participant 08's result from (a) top, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 18:30 mins (top), 15:46 mins (side), and 41:33 mins (upper $45^{\circ}$) drawing without visual scaffold, and 19:21 mins (top), 34:35 mins (side), and 26:01 mins (upper $45^{\circ}$) with visual scaffold.
    }
    \label{fig:result-08}
\end{figure}

\subsection{Chair case2}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub04.pdf}
    \caption{We show participant 04's result from (a) top, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 3:45 mins (top), 4:40 mins (side), and 16:40 mins (upper $45^{\circ}$) drawing without visual scaffold, and 9:00 mins (top), 35:28 mins (side), and 37:00 mins (upper $45^{\circ}$) with visual scaffold.    
    }
    \label{fig:result-04}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub10.pdf}
    \caption{We show participant 10's result from (a) top, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 5:41 mins (top), 4:20 mins (side), and 28:56 mins (upper $45^{\circ}$) drawing without visual scaffold, and 2:37 mins (top), 5:00 mins (side), and 31:19 mins (upper $45^{\circ}$) with visual scaffold.       
    }
    \label{fig:result-10}
\end{figure}

\subsection{Chair case3}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub03.pdf}
    \caption{We show participant 03's result from (a) top, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 19:37 mins (top), 20:39 mins (side), and 43:00 mins (upper $45^{\circ}$) drawing without visual scaffold, and 9:43 mins (top), 15:39 mins (side), and 18:30 mins (upper $45^{\circ}$) with visual scaffold.       
    }
    \label{fig:result-03}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub07.pdf}
    \caption{We show participant 07's result from (a) top, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 08:06 mins (top), 04:19 mins (side), and 48:02 mins (upper $45^{\circ}$) drawing without visual scaffold, and 05:44 mins (top), 03:10 mins (side), and 09:48 mins (upper $45^{\circ}$) with visual scaffold.           
    }
    \label{fig:result-07}
\end{figure}

\subsection{Airplane case1}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub05.pdf}
    \caption{We show participant 05's result from (a) front, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 12:00 mins (front), 08:21 mins (side), and 20:00 mins (upper $45^{\circ}$) drawing without visual scaffold, and 10:30 mins (front), 03:20 mins (side), and 09:56 mins (upper $45^{\circ}$) with visual scaffold.           
    }
    \label{fig:result-05}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub06.pdf}
    \caption{We show participant 06's result from (a) front, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 09:42 mins (front), 11:21 mins (side), and 13:20 mins (upper $45^{\circ}$) drawing without visual scaffold, and 07:46 mins (front), 05:49 mins (side), and 16:47 mins (upper $45^{\circ}$) with visual scaffold.  
    }
    \label{fig:result-06}
\end{figure}
\subsection{Airplane case2}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub02.pdf}
    \caption{We show participant 02's result from (a) front, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 10:21 mins (front), 19:48 mins (side), and 45:47 mins (upper $45^{\circ}$) drawing without visual scaffold, and 18:31 mins (front), 17:10 mins (side), and 16:20 mins (upper $45^{\circ}$) with visual scaffold.  
    }
    \label{fig:result-02}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub09.pdf}
    \caption{We show participant 09's result from (a) front, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 32:28 mins (front), 18:20 mins (side), and 57:12 mins (upper $45^{\circ}$) drawing without visual scaffold, and 17:00 mins (front), 08:54 mins (side), and 41:10 mins (upper $45^{\circ}$) with visual scaffold.  
    }
    \label{fig:result-09}
\end{figure}
\subsection{Airplane case3}
\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub11.pdf}
    \caption{We show participant 11's result from (a) front, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 90:03 mins (front), 15:11 mins (side), and 46:00 mins (upper $45^{\circ}$) drawing without visual scaffold, and 15:00 mins (front), 13:00 mins (side), and 26:12 mins (upper $45^{\circ}$) with visual scaffold.      
    }
    \label{fig:result-11}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/supplemental/sub12.pdf}
    \caption{We show participant 12's result from (a) front, (b) side, and (c) upper $45^{\circ}$ viewpoints.
    The results in the first row are the results without visual scaffold, and the results in second row are the results with visual scaffold.
    This participant spent 39:00 mins (front), 20:10 mins (side), and 16:45 mins (upper $45^{\circ}$) drawing without visual scaffold, and 19:25 mins (front), 24:00 mins (side), and 25:18 mins (upper $45^{\circ}$) with visual scaffold.      
    }
    \label{fig:result-12}
\end{figure}


% \subsection{Participant 1}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub01.pdf}
%     \caption{Caption}
%     \label{fig:result-01}
% \end{figure}
% \subsection{Participant 2}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub02.pdf}
%     \caption{Caption}
%     \label{fig:result-02}
% \end{figure}
% \subsection{Participant 3}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub03.pdf}
%     \caption{Caption}
%     \label{fig:result-03}
% \end{figure}
% \subsection{Participant 4}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub04.pdf}
%     \caption{Caption}
%     \label{fig:result-04}
% \end{figure}
% \subsection{Participant 5}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub05.pdf}
%     \caption{Caption}
%     \label{fig:result-05}
% \end{figure}
% \subsection{Participant 6}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub06.pdf}
%     \caption{Caption}
%     \label{fig:result-06}
% \end{figure}
% \subsection{Participant 7}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub07.pdf}
%     \caption{Caption}
%     \label{fig:result-07}
% \end{figure}
% \subsection{Participant 8}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub08.pdf}
%     \caption{Caption}
%     \label{fig:result-08}
% \end{figure}
% \subsection{Participant 9}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub09.pdf}
%     \caption{Caption}
%     \label{fig:result-09}
% \end{figure}
% \subsection{Participant 10}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub10.pdf}
%     \caption{Caption}
%     \label{fig:result-10}
% \end{figure}
% \subsection{Participant 11}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub11.pdf}
%     \caption{Caption}
%     \label{fig:result-11}
% \end{figure}
% \subsection{Participant 12}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\linewidth]{figs/supplemental/sub12.pdf}
%     \caption{Caption}
%     \label{fig:result-12}
% \end{figure}
